What's in the Box? A Preliminary Analysis of Undesirable Content in the Common Crawl Corpus

Whereas much of the success of the current generation of neural language models has been driven by increasingly large training corpora, relatively little research has been dedicated to analyzing these massive sources of textual data. In this exploratory analysis, we delve deeper into the Common Crawl, a colossal web corpus that is extensively used for training language models. We find that it contains a significant amount of undesirable content, including hate speech and sexually explicit content, even after filtering procedures. We discuss the potential impacts of this content on language models and conclude with future research directions and a more mindful approach to corpus collection and analysis.

==> extras.tex <==
\subsection{Wikipedia}

To give another concrete example, let us turn to Wikipedia, a bastion of free data, often seen as an impartial representation of the current state of human knowledge (which is why we use it to train our language models). However, given the very nature of Wikipedia and its reliance on the contributions of external editors, this brings forward many challenges in terms of verifying all content~\cite{redi2019citation}. In fact, verifiability is one of Wikipedia's core guiding principles, and what makes it impartial and objective. But manually verifying all of its millions or articles is impossible, so developing computational methods is important in order to ensure Wikipedia's impartiality.

While datasets based on Wikipedia such as FEVER~\cite{thorne2018fever} exist and have been used to train computational approaches for fake news detection~\cite{nie2019combining}, these approaches cannot be directly used for actually combating fake news proliferation on Wikipedia. This is due to the fact that, on the one hand, these approaches assume that any provided statements are purely factual (which is not always the case on Wikipedia), and also because the most accurate approaches on datasets such as FEVER are neural network-based and therefore black boxes in terms of explainability. While this works in research, in practice it is necessary to explain why content from Wikipedia is removed and justify moderation to its authors. 

If insights such as these were integrated in the projects working on these challenges and datasets, this could provide orientation to the research directions being pursued and provide motivation to researchers exploring explainable approaches with more varied sources of data. This is even more important given the fact that Wikipedia is extensively used for training models such as BERT~\cite{devlin2018bert} and GPT-3~\cite{brown2020language}, which means that any undetected misinformation can be transferred to black-box models that will use it to both classify and generate further misinformation, potentially amplifying it. 

For instance, the great majority of the architectures and training techniques used for learning word embeddings based are based on the distributional semantics hypothesis, i.e. that words that appear in similar contexts have similar meanings, and will tend to be mapped to vectors that are close together~\cite{mikolov2013efficient}. This, however, is an inadequate measure for representing semantic relations such as synonymy and antonymy (i.e. the vector for `woman' will have a high similarity to both `man' and `female'), and does not represent the distinction between homonyms or polysemes (i.e. 'sign' will have a single vector, whether it means a symbol, the act of writing ones name, etc.) or categories of words (i.e. `bird' and `cat' both belonging to the category `animals')~\cite{rubinstein2015well}. There have been proposals to address these issues, both from the perspective of embeddings themselves~\cite{trask2015sense2vec,cao2017improving} as well as that of similarity calculation~\cite{levy2014linguistic}, but there are many aspects of semantics that these fail to capture. Furthermore, the `analogy' approach used for many bias detection approaches (X is to Y as A is to \rule{0.7em}{0.4pt}) has also been questioned as a way for detecting bias~\cite{nissim2020fair} and merits further analysis. 

